Pyramid Vision Transformer: A Versatile Backbone for Dense Prediction without Convolutions

Although using convolutional neural networks (CNNs) as backbones achieves great successes in computer vision, this work investigates a simple backbone network useful for many dense prediction tasks without convolutions. Unlike the recently-proposed Transformer model (e.g., ViT) that is specially designed for image classification, we propose Pyramid Vision Transformer~(PVT), which overcomes the difficulties of porting Transformer to various dense prediction tasks. PVT has several merits compared to prior arts. (1) Different from ViT that typically has low-resolution outputs and high computational and memory cost, PVT can be not only trained on dense partitions of the image to achieve high output resolution, which is important for dense predictions but also using a progressive shrinking pyramid to reduce computations of large feature maps. (2) PVT inherits the advantages from both CNN and Transformer, making it a unified backbone in various vision tasks without convolutions by simply replacing CNN backbones. (3) We validate PVT by conducting extensive experiments, showing that it boosts the performance of many downstream tasks, e.g., object detection, semantic, and instance segmentation. For example, with a comparable number of parameters, RetinaNet+PVT achieves 40.4 AP on the COCO dataset, surpassing RetinNet+ResNet50 (36.3 AP) by 4.1 absolute AP. We hope PVT could serve as an alternative and useful backbone for pixel-level predictions and facilitate future researches. Code is available at https://github.com/whai362/PVT.

==> table/cls.tex <==
\begin{tabular}{l|c|c|c}
% 	\whline
    %\renewcommand{\arraystretch}{0.7}
	Method & \#Param (M) & GFLOPs & Top-1 (\%)  \\
	\whline
% 	\hline
	R18*~\cite{he2016deep} & 11.7 & 1.8 & 30.2  \\
	R18~\cite{he2016deep}  & 11.7 & 1.8 & 31.5 \\
	DeiT-Tiny/16~\cite{touvron2020training} & \textbf{5.7} & \textbf{1.3} & 27.8 \\
	PVT-Tiny (ours) & 13.2 & 1.9 & \textbf{24.9} \\
	\hline
	R50*~\cite{he2016deep}   &25.6 &4.1 &23.9 \\
	R50~\cite{he2016deep}  &25.6 &4.1 & 21.5 \\
	X50-32x4d*~\cite{xie2017aggregated} &25.0 &4.3 &22.4  \\
	X50-32x4d~\cite{xie2017aggregated} &25.0 &4.3 & 20.5 \\
	DeiT-Small/16~\cite{touvron2020training}  & \textbf{22.1} & 4.6 & \textbf{20.1}
	\\
	PVT-Small (ours)  & 24.5 & \textbf{3.8} & 20.2 \\
	\hline
	R101*~\cite{he2016deep}  &44.7 & 7.9 &22.6\\
	R101~\cite{he2016deep}  &44.7 & 7.9 & 20.2\\
	X101-32x4d*~\cite{xie2017aggregated} & \textbf{44.2} & 8.0 &21.2 \\
	X101-32x4d~\cite{xie2017aggregated} & \textbf{44.2}  & 8.0 & 19.4 \\
	ViT-Small/16~\cite{dosovitskiy2020image} & 48.8 & 9.9 & 19.2 \\
	PVT-Medium (ours) & \textbf{44.2} & \textbf{6.7} & \textbf{18.8}\\
	\hline
	% R152*~\cite{he2016deep} & \textbf{60.2} & 11.6 & 21.7 \\
	% R152~\cite{he2016deep} & \textbf{60.2} & 11.6 \\
	X101-64x4d*~\cite{xie2017aggregated} & 83.5 & 15.6 & 20.4\\
	X101-64x4d~\cite{xie2017aggregated} & 83.5 & 15.6 & 18.5\\
	ViT-Base/16~\cite{dosovitskiy2020image} & 86.6 & 17.6 & \textbf{18.2} \\
	DeiT-Base/16~\cite{touvron2020training} & 86.6 & 17.6 & \textbf{18.2} \\
	PVT-Large (ours) & \textbf{61.4} & \textbf{9.8} & 18.3 \\
% 	\whline
\end{tabular}

==> table/mask.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{l|c|lcc|lcc|lcc|lcc}
% \whline
\multirow{2}{*}{Backbone} & \multirow{2}{*}{\tabincell{c}{\#Param \\(M)}} &\multicolumn{6}{c|}{Mask R-CNN 1x} &\multicolumn{6}{c}{Mask R-CNN 3x + MS} \\
\cline{3-14} 
& &AP$^{\rm b}$ &AP$_{50}^{\rm b}$ &AP$_{75}^{\rm b}$ &AP$^{\rm m}$ &AP$_{50}^{\rm m}$ &AP$_{75}^{\rm m}$ &AP$^{\rm b}$ &AP$_{50}^{\rm b}$ &AP$_{75}^{\rm b}$ &AP$^{\rm m}$ &AP$_{50}^{\rm m}$ &AP$_{75}^{\rm m}$ \\
\whline
% \hline
ResNet18~\cite{he2016deep} & \bf{31.2} & 34.0 & 54.0 & 36.7 & 31.2 & 51.0 & 32.7 & 36.9 & 57.1 & 40.0 & 33.6 & 53.9 & 35.7\\
PVT-Tiny (ours) & 32.9 & \bf{36.7}\gbf{+2.7} & \bf{59.2} & \bf{39.3} & \bf{35.1}\gbf{+3.9} & \bf{56.7} & \bf{37.3} & \bf{39.8}\gbf{+2.9} & \bf{62.2} & \bf{43.0} & \bf{37.4}\gbf{+3.8} & \bf{59.3} & \bf{39.9} \\
\hline
ResNet50~\cite{he2016deep} & 44.2& 38.0 & 58.6 & 41.4 & 34.4 & 55.1 & 36.7 & 41.0 & 61.7 & 44.9 & 37.1 & 58.4 & 40.1\\
PVT-Small (ours) &\bf{44.1} & \bf{40.4}\gbf{+2.4} & \bf{62.9} & \bf{43.8} & \bf{37.8}\gbf{+3.4} & \bf{60.1} & \bf{40.3} & \bf{43.0}\gbf{+2.0} & \bf{65.3} & \bf{46.9} & \bf{39.9}\gbf{+2.8} & \bf{62.5} & \bf{42.8}\\
\hline
ResNet101~\cite{he2016deep} & 63.2 & 40.4 & 61.1 & 44.2 & 36.4 & 57.7 & 38.8 & 42.8 & 63.2 & 47.1 & 38.5& 60.1& 41.3\\
ResNeXt101-32x4d~\cite{xie2017aggregated} &\bf{62.8} & 41.9\gbf{+1.5} & 62.5 & \bf{45.9} & 37.5\gbf{+1.1} & 59.4 & 40.2 & 44.0\gbf{+1.2} & 64.4 & 48.0 & 39.2\gbf{+0.7} & 61.4 & 41.9 \\
PVT-Medium (ours) &63.9 & \bf{42.0}\gbf{+1.6} &\bf{64.4} &45.6 &\bf{39.0}\gbf{+2.6}& \bf{61.6}& \bf{42.1} & \bf{44.2}\gbf{+1.4} & \bf{66.0} & \bf{48.2} & \bf{40.5}\gbf{+2.0} & \bf{63.1} & \bf{43.5}\\
\hline
ResNeXt101-64x4d~\cite{xie2017aggregated} &101.9 & 42.8 & 63.8 & \bf{47.3} & 38.4 & 60.6 & 41.3 & 44.4 & 64.9 & 48.8 & 39.7& 61.9 & 42.6 \\
PVT-Large (ours) &81.0 & \bf{42.9}\gbf{+0.1}& \bf{65.0} & 46.6 &\bf{39.5}\gbf{+1.1}& \bf{61.9}& \bf{42.5} \\
% \whline
\end{tabular}

==> table/retina.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{l|c|lcc|ccc|lcc|ccc}
% \whline
\multirow{2}{*}{Backbone} & \multirow{2}{*}{\tabincell{c}{\#Param \\(M)}} &\multicolumn{6}{c|}{RetinaNet 1x} &\multicolumn{6}{c}{RetinaNet 3x + MS} \\
\cline{3-14} 
& &AP &AP$_{50}$ &AP$_{75}$ &AP$_S$ &AP$_M$ &AP$_L$ &AP &AP$_{50}$ &AP$_{75}$ &AP$_S$ &AP$_M$ &AP$_L$ \\
\whline
% \hline
ResNet18~\cite{he2016deep} &\bf{21.3} & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2 & 35.4 & 53.9 & 37.6 & 19.5 & 38.2  &46.8 \\
PVT-Tiny (ours) &23.0& \bf{36.7}\gbf{+4.9}& \bf{56.9}& \bf{38.9}& \bf{22.6}& \bf{38.8} &\bf{50.0} & \bf{39.4}\gbf{+4.0} & \bf{59.8} & \bf{42.0} & \bf{25.5} & \bf{42.0} & \bf{52.1} \\
\hline
ResNet50~\cite{he2016deep} &37.7 & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8 & 39.0 & 58.4 & 41.8 & 22.4 & 42.8 & 51.6  \\
PVT-Small (ours) & \bf{34.2} & \bf{40.4}\gbf{+4.1} & \bf{61.3} & \bf{43.0} & \bf{25.0} & \bf{42.9} & \bf{55.7} & \bf{42.2}\gbf{+3.2} & \bf{62.7} & \bf{45.0} & \bf{26.2} & \bf{45.2} & \bf{57.2 }\\
\hline
ResNet101~\cite{he2016deep} &56.7  & 38.5 & 57.8 & 41.2 & 21.4 & 42.6 & 51.1 & 40.9 & 60.1 & 44.0 & 23.7 & 45.0 & 53.8
\\
ResNeXt101-32x4d~\cite{xie2017aggregated} &56.4& 39.9\gbf{+1.4} & 59.6 & 42.7 & 22.3 & 44.2 & 52.5 & 41.4\gbf{+0.5} & 61.0 & 44.3 &23.9& 45.5 & 53.7 \\
PVT-Medium (ours) &\bf{53.9} & \bf{41.9}\gbf{+3.4} & \bf{63.1} & \bf{44.3} & \bf{25.0} & \bf{44.9} & \bf{57.6} & \bf{43.2}\gbf{+2.3} & \bf{63.8} & \bf{46.1} & \bf{27.3} & \bf{46.3} & \bf{58.9}\\
\hline
ResNeXt101-64x4d~\cite{xie2017aggregated} & 95.5& 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0 & 41.8& 61.5 & 44.4 & 25.2& 45.4& 54.6 \\
PVT-Large (ours) & 71.1 & \bf{42.6}\gbf{+1.6} & \bf{63.7} & \bf{45.4} & \bf{25.8} & \bf{46.0} & \bf{58.4}
 \\
% \whline
\end{tabular}

==> table/seg.tex <==
\begin{tabular}{l|c|l}
% 	\whline
	Backbone & \multicolumn{2}{c}{Semantic FPN}\\
	\cline{2-3}
	& \#Param (M) & mIoU (\%)   \\
	\whline
% 	\hline
	ResNet18~\cite{he2016deep} & \bf{15.5} & 32.9 \\
	PVT-Tiny (ours) & 17.0 & \bf{35.7}\gbf{+2.8} \\
	\hline
ResNet50~\cite{he2016deep} & 28.5 & 36.7\\
PVT-Small (ours) & \bf{28.2}& \bf{39.8}\gbf{+3.1}\\
\hline
ResNet101~\cite{he2016deep} & 47.5& 38.8\\
ResNeXt101-32x4d~\cite{xie2017aggregated} & \bf{47.1} & 39.7\gbf{+0.9} \\
PVT-Medium (ours) & 48.0 & \bf{41.6}\gbf{+2.8}\\
\hline
ResNeXt101-64x4d~\cite{xie2017aggregated} & 86.4 & 40.2\\
PVT-Large (ours) & \textbf{65.1} & \bf{42.1}\gbf{+1.9} \\
% 	\whline
\end{tabular}
